Constrained High Dimensional Statistical Inference

In typical high dimensional statistical inference problems, confidence intervals and hypothesis tests are performed for a low dimensional subset of model parameters under the assumption that the parameters of interest are unconstrained. However, in many problems, there are natural constraints on model parameters and one is interested in whether the parameters are on the boundary of the constraint or not. e.g. non-negativity constraints for transmission rates in network diffusion. In this paper, we provide algorithms to solve this problem of hypothesis testing in high-dimensional statistical models under constrained parameter space. We show that following our testing procedure we are able to get asymptotic designed Type I error under the null. Numerical experiments demonstrate that our algorithm has greater power than the standard algorithms where the constraints are ignored. We demonstrate the effectiveness of our algorithms on two real datasets where we have {\emph{intrinsic}} constraint on the parameters.

==> Multidimension.tex <==
\section{Multidimensional Test} \label{sec:multidimension}

%Up to now we have focused on testing for scalar $\alpha$. In this section we generalize our algorithm to multivariate case. We now have the partition $\bm \beta = (\bm{\alpha} , \bm{\theta})$ with $d$ dimensional parameter of interest $\bm{\alpha}$, and $p-d$ dimensional nuisance parameter $\bm \theta$ where we assume $d \ll p$. 
%The hypothesis we want to test is $H_0: \alpha_1^* = ... = \alpha^*_d = 0$ versus $H_A: \exists i\in \{1,...,d\} \,\,\, s.t. \, \,\,\alpha_i^* > 0$. 
%The algorithm is very similar to the one dimensional case. Specifically, in Step 1, the vector $\bm{\hat w}$ is replaced by a matrix $\hat{\bm{W}} \in \mathbb R^{(p-d) \times d}$ and $\hat{\bm{W}}$ can be calculated column-wise: for each $j=1, ..., d$ we can solve for $\bm{\hat w}_j$ as in Step 1, and combine them to get matrix $\hat{\bm{W}}$, i.e., $\hat{\bm{W}} = (\hat{\bm w}_1, ... , \hat{\bm w}_d)$ where
%\begin{gather}
%\hat{\bm w}_j = \text{argmin}_{\bm w} \|\bm w\|_1, \notag \\
%\text{ s.t. } \| \nabla^2_{\alpha_j\bm \theta}\ell(\widehat{\bm \beta}) - \bm w^T \nabla^2_{\bm \theta\bm \theta}\ell(\widehat{\bm \beta}) \|_{\infty} \leq \lambda'. \notag
%\end{gather}
%The decorrelated score function, decorrelated estimator and decorrelated likelihood function all remain the same, with $\hat{\bm w}$ replaced by $\hat{\bm{W}}$:
%\begin{gather}
%\hat{\bm U}(\bm \alpha,\hat{\bm \theta}) = \nabla_{\bm \alpha}\ell(\bm \alpha, \hat{\bm \theta}) - \hat{\bm{W}}^T \nabla_{\bm \theta}\ell(\bm \alpha, \hat{\bm \theta}), \notag \\
%\tilde{\bm \alpha} = \hat{\bm \alpha} - \Big(\frac{\partial\hat{\bm U}(\hat{\bm \alpha}, \hat{\bm \theta})}{\partial \bm \alpha}\Big)^{-1} \cdot \hat{\bm U}(\hat{\bm \alpha}, \hat{\bm \theta}),\notag \\
%\ell_{\text{de}}(\bm \alpha) = \ell(\bm \alpha,\bm{\hat \theta} - \bm{\hat W}\bm \alpha). \notag
%\end{gather}
%Here $\hat{\bm U}(\bm \alpha,\hat{\bm \theta})$ and $\tilde{\bm \alpha}$ are both $d$ dimensional vectors. The asymptotic normality of decorrelated score function and estimator still holds:
%\begin{gather}
%\sqrt{n}\hat{\bm U}(\bm 0,\hat{\bm \theta}) \overset{d}{\to} N(\bm 0, H_{\bm \alpha | \bm \theta}), \notag \\
%\sqrt{n} \tilde{\bm \alpha} \overset{d}{\to} N(\bm 0, H_{\bm \alpha | \bm \theta}^{-1}), \notag
%\end{gather}
%where $H_{\bm \alpha | \bm \theta} = H_{\bm \alpha\bm \alpha}^* - H_{\bm \alpha\bm \theta}^*{H_{\bm \theta\bm \theta}^{*-1}}H_{\bm \theta\bm \alpha}^*$, and again it can be estimated by sample version $\hat H_{\bm \alpha | \bm \theta}$. Step 2 is also the same as before, except in vector form. Finally, under the null hypothesis, the asymptotic distribution of $T_s$, $T_w$ and $T_L$ are still mixed $\chi^2$:
%$$
%T_s, T_w, T_L \overset{d}{\to} \sum_{i=1}^d w_i \chi^2_i.
%$$









%Unlike scalar case, the weights here are much more complicated. For notation simplicity we use $\bm V$ to denote $ H_{\bm \alpha|\bm \theta}^{-1}$. In \cite{kudo1963multivariate} the authors show that the weights should be:
%\begin{equation}
%w_i = \sum_{|\eta| = i} p\Big\{ (\bm V_{\eta'})^{-1} \Big\} \cdot p\Big\{ \bm V_{\eta;\eta'} \Big\},
%\label{wi}
%\end{equation}
%where the summation runs over all subsets $\eta$ of $\{1, ..., d\}$ having $i$ element. $\eta'$ is the complement of $\eta$ and $\bm V_{\eta}$ is the submatrix of $\bm V$ corresponding to those $y_i$ where $i \in \eta$. $\bm V_{\eta;\eta'}$ is the covariance matrix under the condition $y_j = 0$ where $j \in \eta'$. Finally $p(\bm \Lambda)$ denotes the probability that $\bm z \geq 0$ for a Gaussian random variable $\bm z \sim N(\bm 0, \bm \Lambda)$.

One exception is when these variables are independent (i.e., $\bm V$ is a diagonal matrix). In this case the weights are given by:
\begin{equation}
w_i = 2^{-d}\binom{d}{i}.
\end{equation}
The main theorem for multidimensional case is similar to one dimensional case. Now we are jointly testing $d$ parameters, $H_0: \alpha_1^* = ... = \alpha^*_d = 0$ versus $H_A: \exists i \in \{1,...,d\} \,\,\, s.t. \, \,\,\alpha_i^* > 0$. We have the following theorem:

\begin{theorem}
Suppose all the conditions hold, the test statistics $T_s$, $T_w$ and $T_L$ constructed in Step 2 for multidimensional case have asymptotic distribution $\sum_{i=1}^d w_i \chi^2_i$ under the null, where $\chi_0^2$ is point mass at $0$, and the weights $w_i$ are given by \eqref{wi} with $\bm V = H_{\bm \alpha|\bm \theta}^{-1}$.
\label{main}
\end{theorem}


With this mixed Chi-square distribution under the null, we can build hypothesis testing for $\bm \alpha^*$ as before. The critical value can be calculated by numerical methods.



\subsection{Proof of Theorem \ref{main}}

%Now since we have the asymptotic normality for $\widehat{U}(0,\widehat{\bm \theta})$ and $\tilde \alpha$, we then calculate the one-sided score, wald and likelihood ratio test statistic according to Step 2. For Theorem 4 and Theorem 5, we first focus on $T_s$ and $T_w$, and give an intuitive proof for the following more general claim.

Before we proceed with the main proof, we first introduce the following lemmas.


\vspace{1mm}
\begin{lemma}
Suppose $\bm Y \sim N(\bm 0,\bm V)$ is a $d$ dimensional normal variable, define
\begin{equation}
T = \bm Y^T\bm V^{-1}\bm Y - \inf_{\bm  b \geq 0}{\Big\{(\bm Y-\bm b)^T\bm V^{-1}(\bm Y-\bm b) \Big\}}.
\end{equation}
Then $T$ is distributed as a mixture of Chi-square distribution with the weights given in \eqref{wi}.
\label{lemma_mix}
\end{lemma}
\begin{proof}
We rewrite $T$ as
\begin{equation}
\begin{aligned}
T & = \big(\bm V^{-\frac 12}\bm Y\big)^T \big(\bm V^{-\frac 12}\bm Y\big) \\
& \quad - \inf_{\bm b \geq 0}{\Big\{\big(\bm V^{-\frac 12}\bm Y-\bm V^{-\frac 12}\bm b\big)^T\big(\bm V^{-\frac 12}\bm Y-\bm V^{-\frac 12}\bm b\big) \Big\}} \\
& = \Big\| \bm V^{-\frac 12}\bm Y \Big\|_2^2 - \inf_{\bm b \geq 0}{\Bigg\{\Big\|\bm V^{-\frac 12}\bm Y-\bm V^{-\frac 12}\bm b\Big\|_2^2 \Bigg\}}.\\
\end{aligned}
\end{equation}
Since $\bm V^{-\frac 12}\bm Y \sim N(\bm 0,\bm I_d)$, we can directly apply the results in \cite{kudo1963multivariate} and obtain
%In the second term, some of them are canceled by $\bm V^{-\frac 12}\bm b$. Those who are not canceled by $\bm V^{-\frac 12}\bm b$ gives the same value as the first term, so they canceled; while those who are canceled by $\bm V^{-\frac 12}\bm b$ gives 0 and then the first term remains. In all $T$ is the summation of some square of i.i.d $N(0,1)$ normal variables. Each of them have the weight corresponding to the probability that certain number of elements are canceled by $\bm V^{-\frac 12}\bm b$. So we have
\begin{equation}
\text{Pr}(T \geq c) = \sum_{i=0}^p w_i \cdot \text{Pr}(\chi^2_i \geq c)
\end{equation}
for any $c$ with the weights given in \eqref{wi}, which demonstrates the mixed Chi-square distribution.

%The weight $w_i$ depends on $p$ and $\bm V$: $w_i = w_i(p,\bm V)$. The computation may be difficult for relatively large $p$. Kudo (1963) \cite{kudo1963multivariate} showed that the weight is the following:
%$$
%w_i(p,\bm V) = \sum_{|\alpha| = i} p\big\{ (\bm V_{\alpha'})^{-1} \big\} \cdot p\big\{ \bm V_{\alpha;\alpha'} \big\}
%$$
%where the summation runs over all subsets $\alpha$ of $\{1, ..., p\}$ having $i$ element. $\alpha'$ is the complement of $\alpha$, $\bm V_{\alpha}$ is the submatrix of $\bm V$ corresponding to those $y_i$ ($i \in \alpha$). $\bm V_{\alpha;\alpha'}$ is the covariance matrix under the condition $y_j = 0$ ($j \in \alpha'$). Finally $p(\bm \Lambda)$ denotes the probability that $\bm z \geq 0$ for a normal variable $\bm z \sim N(\bm 0, \bm \Lambda)$.

For large $d$ the calculation of weights can be computational intensive and is usually performed using numerical methods. One exception is when $\bm V = \bm I_d$, where we have $\bm Y \sim N(\bm 0,\bm I_d)$ and we can rewrite $T$ as
\begin{equation}
\begin{aligned}
T & = \bm Y^T\bm Y - \inf_{\bm b \geq 0}{\Big\{(\bm Y-\bm b)^T(\bm Y-\bm b) \Big\}}\\
& = \sum_{i=1}^p \max{(y_i,0)}^2.
\end{aligned}
\end{equation}
Now each term in the summation is the mixture of $\chi_0^2$ and $\chi_1^2$ with probability half and half. Hence the distribution of $T$ is the convolution:
\begin{equation}
\Big( \frac 12 \chi^2_0 + \frac 12 \chi^2_1 \Big)^{*d} = \frac{1}{2^d}\sum_{i=0}^d \binom{d}{i} \chi_i^2,
\end{equation}
and therefore the weight $w_i$ is
\begin{equation}
2^{-d}\binom{d}{i}.
\end{equation}
Particularly for one dimensional case it is just
\begin{equation}
\frac 12 (\chi^2_0 +  \chi^2_1).
\end{equation}
\end{proof}


\begin{proof}[Proof of Theorem \ref{main}]
From the procedure we see that $\hat{\bm W}$ is constructed column-wise. 
Following the same outline in the proofs of Lemma \ref{lemma_normal} and Lemma \ref{lemma_consistency} we have the following asymptotic distributions under the null:
\begin{gather}
\sqrt{n}\hat{\bm U}(0,\hat{\bm \theta}) \overset{d}{\to} N(0, H_{\bm \alpha | \bm \theta}), \notag \\
\sqrt{n} \tilde{\bm \alpha} \overset{d}{\to} N(0, H_{\bm \alpha | \bm \theta}^{-1}), \notag
\end{gather}
and the consistency of the estimator $\hat H_{\bm \alpha | \bm \theta}$. Lemma \ref{lemma_mix} then ensures that the asymptotic distributions of $T_s$ and $T_w$ are mixed Chi-square.
%First we have the multivariate Central Limit Theory, particularly for i.i.d case, and then we have $d$ dimensional $\hat{\bm U}$ and $\tilde{\bm \alpha}$. All the procedures and proofs follow column-wisely. The proof of the asymptotic mixed $\chi^2$ distribution is in the Appendix.



We then turn to $T_L$. %Having the above theorem, we can see that $T_w$ and $T_s$ have the asymptotic $\chi^2$ distribution. While for the likelihood ratio test statistic $T_L$, 
According to the proof of Theorem 4.9 in \cite{fang2014testing}, under the null we have
\begin{equation}
\begin{aligned}
T_L & = -2n\Big(\tilde \nu^T\hat U(0, \hat{\bm \theta}) + \frac{1}{2}\tilde \nu^T \hat H_{\alpha|\bm \theta} \tilde \nu\Big)  + o_{\mathbb P}(1)\\
& = -2n\Big(-\tilde \nu^T\hat H_{\alpha|\bm \theta}\tilde \alpha+\frac12 \tilde \nu^T  \hat H_{\alpha|\bm \theta} \tilde \nu\Big) + o_{\mathbb P}(1)\\
& = n\Big( \tilde \alpha^T\hat H_{\alpha|\bm \theta}\tilde \alpha - (\tilde \alpha -\tilde \nu)^T\hat H_{\alpha|\bm \theta}(\tilde \alpha -\tilde \nu)\Big) + o_{\mathbb P}(1) \\
& = T_w + o_{\mathbb P}(1).
\end{aligned}
\end{equation}

Therefore $T_L$ has the same asymptotic distribution as $T_w$.

\end{proof}

%With this null distribution we could construct test for $H_0 : \bm{\alpha} = 0$. Given the desired Type I error $\gamma$, we can calculate the $\gamma$ quantile of the distribution by numeric method, and we reject $H_0$ when $T_s$, $T_w$ or $T_L$ is greater than that critical value. This is our desired test, with asymptotic Type I error $\gamma$. 







